MOT16: A Benchmark for Multi-Object Tracking

Standardized benchmarks are crucial for the majority of computer vision applications. Although leaderboards and ranking tables should not be over-claimed, benchmarks often provide the most objective measure of performance and are therefore important guides for reseach. Recently, a new benchmark for Multiple Object Tracking, MOTChallenge, was launched with the goal of collecting existing and new data and creating a framework for the standardized evaluation of multiple object tracking methods. The first release of the benchmark focuses on multiple people tracking, since pedestrians are by far the most studied object in the tracking community. This paper accompanies a new release of the MOTChallenge benchmark. Unlike the initial release, all videos of MOT16 have been carefully annotated following a consistent protocol. Moreover, it not only offers a significant increase in the number of labeled boxes, but also provides multiple object classes beside pedestrians and the level of visibility for every single object of interest.

==> biographies.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{biography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{laura.jpg}}]{Laura Leal-Taixe{\'e}}
received her Bachelor and Master degrees in Telecommunications Engineering from the Technical University of Catalonia (UPC), Barcelona. In 2008 she did her Master Thesis at Northeastern University, Boston, USA and in 2014 she received her PhD degree (Dr.-Ing.) from the Leibniz University Hannover, Germany. During her PhD she did a one-year visit at the Vision Lab at the University of Michigan, USA. She is currently a postdoctoral researcher at the Institute of Geodesy and Photogrammetry of ETH Zurich, Switzerland. 
Her research interests are multiple object tracking, with special focus on social motion models and global optimization methods, as well as scene understanding.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{anton.jpg}}]{Anton Milan}
(n{\'e} Andriyenko) received his Diplom degree in Computer Science (Dipl.-Inform.) from the University of Bonn in 2008. He has worked as a software developer in the computer graphics industry. Here received his PhD in 2013 from the Technical University Darmstadt, Germany, after which he visited the PRML group at the Hokkaido University in Japan. Since 2014, he is a post-doctoral researcher at the Australian Centre for Visual Technologies (ACVT) at the University of Adelaide. His research interests are energy-based optimization methods for real-world multiple people tracking scenarios.
\end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ian.jpg}}]{Ian Reid}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{stefan.jpg}}]{Stefan Roth}
received the Diplom degree in Computer Science and Engineering from the University of Mannheim, Germany in 2001. In 2003 he received the MSc degree in Computer Science from Brown University, and in 2007 the PhD degree in Computer Science from the same institution. Since 2007 he is an assistant professor of Computer Science at Technical University Darmstadt, Germany. His research interests include probabilistic and statistical approaches to image modeling, motion estimation,
human tracking, and object recognition. He received several awards, including an honorable mention for the Marr Prize at ICCV 2005 (with M. Black), the Olympus-Prize 2010 of the German Association for Pattern Recognition (DAGM) and the Heinz Maier-Leibnitz Prize 2012 of the German Research Foundation (DFG). He serves on the editorial board of the International Journal of Computer Vision (IJCV).
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{konrad.jpg}}]{Konrad Schindler}
received a Diplomingenieur (M.tech) degree in photogrammetry from Vienna University of Technology, Austria in 1999, and a PhD from Graz University of Technology, Austria, in 2003. He has worked as a photogrammetric engineer in the private industry, and held researcher positions in the Computer Graphics and Vision Department of Graz University of Technology, the Digital Perception Lab of Monash University, and the Computer Vision Lab of ETH Zurich. He became assistant professor of Image Understanding at TU Darmstadt in 2009, and since 2010 has been a tenured professor of Photogrammetry and Remote Sensing at ETH Zurich. His research interests lie in the field of computer vision, photogrammetry, and remote sensing, with a focus on image understanding and 3d reconstruction. He currently serves as head of the Institute of Geodesy and Photogrammetry, and as associate editor for the ISPRS Journal of Photogrammetry and Remote Sensing, and for the Image and Vision Computing Journal.
\end{IEEEbiography}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}


==> submission.tex <==
\section{Benchmark Submission}
\label{sec:benchmark-structure}
Our benchmark consists of the database and evaluation server on one hand, 
and the website as the user interface on the other. It is open to 
everyone who respects the submission policies (see next section). Before 
participating, every user is required to create an account providing
an institutional (as opposed to a generic) e-mail
address\footnote{For accountability and to prevent abuse by using several email accounts.}. 
After registering, the user can create a 
new tracker with a unique name and enter all additional details. It is 
mandatory to indicate
\begin{itemize}
\item the challenge or benchmark category in which the tracker will be 
participating,
%
\item the full name and a brief description of the method including the parameters used,

\item whether the method operates online or on a 
batch of frames and whether the source code is publicly available,

\item the \emph{total} runtime in seconds for computing the results on all 
sequences and the hardware used, and 
%
\item whether only the provided or also external training and detection 
data were used. 

%
\end{itemize}
%

%


After entering all details, it is possible to submit the results in 
the format described in \Sec~\ref{sec:data-format}. The tracking 
results will be automatically evaluated and appear on the user's profile. 
They will \emph{not} be displayed in the public ranking table. 
The user can then decide at any point in time to 
make the results public. Note that the results can be published anonymously,
\eg to enable a blind review process for a corresponding paper. In this case,
we ask to provide the venue and the paper ID or a similar unique reference.
We request that a proper reference to the method's description is added 
upon acceptance of the paper. In case of rejection, an anonymous entry may 
also be removed from the database. Anonymous entries will also be removed
after six months of inactivity.

The tracker's meta information such as description, or project page can be edited
at any time. Visual results of all public submissions, as well as annotations and
detections can be viewed on a dedicated 
visualization page.\footnote{\url{http://motchallenge.net/vis/}}



\subsection{Submission policy}
The main goal of this benchmark is to provide a platform that allows for 
an objective performance comparison of multiple target tracking 
approaches on real-world data. Therefore, we introduce a few simple 
guidelines that must be followed by all participants.

{\bf Training.} Ground truth is only provided for the training sequences.
It is the participant's own responsibility to find the best setting
using \emph{only} the training data.
The use of additional training data must be indicated during submission and will
be visible in the public ranking table.
The use of ground truth labels on the test data is strictly forbidden. This or any other misuse
of the benchmark will lead to the deletion of the participant's account and their results.

{\bf Detections.} We also provide a unique set of detections 
(see \Sec \ref{sec:detections}) for each sequence. We highly encourage all tracking-by-detection
algorithms to use the given detections. In case the user wants to present results with another set of
detections or is not using detections at all, this should be clearly stated during submission
and will also be displayed in the results table.
 
 {\bf Variations of the same tracker.} Each method corresponds to a single tracker created in the benchmark.
 Variations of the same method, \eg different features used, can only be evaluated on the training data.
 

{\bf Submission frequency.} Generally, we expect one single submission 
for every tracking approach. If for any reason, the user needs to 
re-compute and re-submit the results (\eg due to a bug discovered in the 
implementation), he/she may do so after a waiting period of 72 hours 
after the last submission. This policy should discourage the use of the
benchmark server for training and parameter tuning on the test data. The maximum number of
submissions per method is 4.
%
Under \emph{no} circumstances must anyone create a second account and 
attempt to re-submit in order to bypass the waiting period. This may lead
to a deletion of the account and excluding the user from participating
in the benchmark.

